Knowledge Tracing: A Survey

Humans ability to transfer knowledge through teaching is one of the essential aspects for human intelligence. A human teacher can track the knowledge of students to customize the teaching on students needs. With the rise of online education platforms, there is a similar need for machines to track the knowledge of students and tailor their learning experience. This is known as the Knowledge Tracing (KT) problem in the literature. Effectively solving the KT problem would unlock the potential of computer-aided education applications such as intelligent tutoring systems, curriculum learning, and learning materials' recommendation. Moreover, from a more general viewpoint, a student may represent any kind of intelligent agents including both human and artificial agents. Thus, the potential of KT can be extended to any machine teaching application scenarios which seek for customizing the learning experience for a student agent (i.e., a machine learning model). In this paper, we provide a comprehensive and systematic review for the KT literature. We cover a broad range of methods starting from the early attempts to the recent state-of-the-art methods using deep learning, while highlighting the theoretical aspects of models and the characteristics of benchmark datasets. Besides these, we shed light on key modelling differences between closely related methods and summarize them in an easy-to-understand format. Finally, we discuss current research gaps in the KT literature and possible future research and application directions.

==> background.tex <==
\section{BACKGROUND}
\label{Sec:BA}
\q{(Discuss: I'm not sure about this section - both structure and content. Generally, it reads a bit loose-fitting.)} In this Section, we provide a detailed introduction for the theoretical background concepts related to the methods reviewed in this survey. We start by introducing the concept of intelligent tutoring systems as the main niche for knowledge tracing methods. Then, we introduce concepts of the learning curve theory illustrating the knowledge retention and forgetting forces in humans. Finally, we outline the main sequence modelling concepts utilized as building blocks in recent knowledge tracing literature.



\subsection{Intelligent Tutoring Systems (ITSs)}
\q{(Suggestion: delete this subsection)} An intelligent tutoring system (ITS) aims at providing customized learning guidance to students without intervention from human teachers~\cite{psotka1988intelligent,rathore2020intelligent}. 
It is a vital success factor for any ITS to have an effective knowledge tracing capability in order to provide a similar learning experience that a human teacher can provide for students ~\cite{corbett1994knowledge,piech2015deep,desmarais2012review,ChenLHWCWSH17,ktfm19}.

\subsection{The Learning Curve Theory}
\q{(discuss: this reads more specific to memory and forgetting - so should be moved to somewhere close to forgetting)} Attempts to understand the memory working mechanisms in the human brain go back to almost a century ago with the work done by Hermann Ebbinghaus~\cite{ebbinghaus2013memory,repeat_ebbinghouse_15}, who studied forces that affect information retention from an experimental psychology perspective to formulate what is currently known as the learning curve theory~\cite{learning_curve_theory}. There are two effects that are reflecting these forces on memory retention and retrieval namely the \emph{forgetting} effect and the \emph{learning} effect. The former is reflecting the decay of memory retention over time, Ebbinghaus indicated that this decay over time follows an exponential decay pattern as shown in Equation~\ref{eq:ebbing_forget}:

\begin{equation}
R = e^{-\frac{t}{S}}
    \label{eq:ebbing_forget}
\end{equation}

\noindent where $R$ is the information retention rate, $t$ is the time steps passed since being firstly introduced to the information, and $S$ is the memory stability in holding learned information in lack of revision and practice over time.

While the learning effect works as an opposite force against forgetting through repeated revision and practice of the learned information. Figure~\ref{fig:forgetting_curve} shows this interplay between forgetting and learning effects over time.

\begin{figure}[H]
\centering
\includegraphics[width=0.65\textwidth]{figs/Ebbinghaus-forgetting-curve-and-review-cycle.png}
\caption{Ebbinghaus forgetting curve over time with and without the impact of reviewing the learned information~\cite{Forget_fig}.}
\label{fig:forgetting_curve}
\end{figure}

Tracing the knowledge state of a student without counting for the impact of forgetting effect could lead to a significant error in the estimate and thus mislead the actions taken by an intelligent teaching strategy. Modelling the forgetting effect during knowledge tracing is one of the major challenges that relevant literature aimed at tackling, we introduce these attempt in detail in Section~\ref{sec:RW}.

\subsection{Sequence Modelling}
\q{(discuss: no need to discuss the standard NN models in this survey for KT - need to cut and then incorporate some bits into other related parts)}
The knowledge tracing task can be represented through a sequence prediction objective from a machine learning perspective. That is given the previous sequence of question answering, we need to predict the probability of answering the current question correctly. Following this representation, it is necessary to introduce some of the main sequence modelling building blocks that appear in the knowledge tracing literature. Over the last decade, deep neural network models achieved major breakthroughs in sequence modeling applications~\citep{SCHMIDHUBER201585,NIPS2014_5346,Graves2013,2013arXiv1308.0850G}. This made many knowledge tracing methods to adopt them for representing and modelling the temporal dynamics in a student's knowledge state. In this section, we provide an overview of the different types of deep neural networks related to sequence modeling.

Conventional neural networks assume that the input samples are independent and identically distributed (iid)~\citep{statIndepence90}, which is a valid assumption with non-temporal data scenarios (e.g., classifying images of cats and dogs). However, sequence data does not satisfy this assumption as the latest input observation will be dependent on the previous history of the sequence. For example, consider a sentiment analysis task~\citep{INR-011}, in which we need to understand a human's opinion from a paragraph of text, we cannot deal with each word separately to achieve such objective. Similarly, in the KT scenario, we cannot assume that a student's answers are independent of each other as the probability of answering the latest exercise will be dependent on the performance on answering previous relevant exercises reflecting her knowledge state across the involved knowledge components in the task. 

Recurrent neural networks (RNNs) do not assume that the input samples are iid and consider previous sequence information when dealing with a new observation. Thus, this model takes the latest observation and combine it with an internal state summarizing previous observations. This recurrence gives RNNs a form of memory that can hold important information on the sequence level.

\begin{figure}[H]
\centering
\includegraphics[width=0.55\textwidth]{figs/RNN.jpg}
\caption{A recurrent neural network and its unfolding over time.}
\label{fig:RNN}
\end{figure}
Figure~\ref{fig:RNN} illustrates a recurrent neural network. The variable $\mathit{i}$ represents an input (e.g., a one-hot encoding vector representing the current word in the sequence , the variable $\mathit{h}$ represents the network's hidden state, and the variable $\mathit{g}$ represents the network's output (e.g., probability of the next word in the sequence). The learning parameters $\mathit{W_{\mathit{i}}}$, $\mathit{W_{\mathit{h}}}$, and $\mathit{W_{\mathit{g}}}$ represent the weight vectors for the input, hidden state, and output respectively. The hidden state and output are calculated as follows:

\begin{equation}
    \label{eq:RNN}
   {h_{t}=\sigma(W_{i}\cdot i_{t}+W_{h}\cdot h_{t-1})}
\end{equation}
\begin{equation}
    \label{eq:RNN}
   {g_{t}=Softmax(W_{g}\cdot h_{t})}
\end{equation}

\noindent where $\sigma(i)=\frac{1}{1+e^{-i}}$ and $Softmax(i_{k})=\frac{e^{i}k}{\sum_{j=0}^{k}e^{i}j}$ are activation functions. \\   
 
Despite the effectiveness of RNNs in modeling sequence dynamics, they suffer from the vanishing gradient issue over long sequences as their internal state is updated in each time step~\citep{LEVIN1990641,pascanu2013difficulty}. To overcome this limitation, long short-term memory networks were introduced~\citep{LSTM}. LSTM has two hidden states instead of one in the RNN in addition to three gates that control the update of the hidden state, thus it is not completely updated in each time step as in RNNs. 
\begin{figure}[H]
\centering
\includegraphics[width=0.55\textwidth]{figs/lstm_cell.pdf}
\caption{A visual representation for the design of an LSTM cell. }
\label{fig:LSTM}
\end{figure}

The LSTM cell has three gates $I_{t},F_{t}$, and $O_{t}$ in addition to two states $h_{t}$ and $v_{t}$. The input gate $I_{t}$ determines how much information from the current input $g_{t}$ is going to affect the current cell's state $c_{t}$. The forget gate $F_{t}$ decides what information should be forgotten or kept from the current input $g_{t}$ and the previous cell's state $c_{t-1}$. While the output gate $o_{t}$ controls which information from the current cell's state $c_{t}$ should flow to the current hidden state $h_{t}$. The cell's state $c_{t}$ stores long and short-term information about the sequence. While the hidden state $h_{t}$ is the cell's output with respect to the current input $g_{t}$, the current cell's state $c_{t}$, and the previous hidden state $h_{t-1}$. Figure \ref{fig:LSTM} depicts the design of the LSTM cell. The corresponding equations for the LSTM cell are presented as follows: 

\begin{equation}
{I_{t}=\sigma(\mathbf{W_{\mathrm{i}}\mathrm{[h_{t-1},g_{t}]+b_{i})}}}
\end{equation}
\begin{equation}
{F_{t}=\sigma(\mathbf{W_{\mathrm{f}}\mathrm{[h_{t-1},g_{t}]+b_{f})}}}
\end{equation}
\begin{equation}
{O_{t}=\sigma(\mathbf{W_{\mathrm{o}}\mathrm{[h_{t-1},g_{t}]+b_{o})}}}
\end{equation}
\begin{equation}
{\tilde{c}_{t}}=\mathrm{Tanh}(\mathbf{W_{\mathrm{c}}\mathrm{[h_{t-1},g_{t}]+b_{c})}}
\end{equation}
\begin{equation}
{c_{t}}=\mathrm{F_{t}\odot c_{t-1}+I_{t}\odot\tilde{c}_{t}}
\end{equation}
\begin{equation}
{h_{t}=O_{t}\odot Tanh(c_{t})}
\end{equation}\\

\noindent where $\sigma(i)=\frac{1}{1+e^{-i}}$ and ${Tanh(u_{i})=(e^{u_{i}}-e^{-u_{i}})/(e^{u_{i}}+e^{-u_{i}})}$ are activation functions.\\ 

A more computationally efficient variant of LSTMs is gated recurrent unit (GRU), that aims at speeding up the training of the cell while preserving the same performance level~\citep{2014arXiv1412.3555C}. Figure~\ref{fig:GNN} shows a modular design for a gated recurrent unit. Instead of three gates as in LSTM cells, GRUs have only two gates. First, the update gate $z_{t}$ which decides the magnitude of the update on the hidden state based on the input and the past hidden state value. Second the reset gate $r_{t}$ which is considered the opposite of the previous gate is responsible for deciding on the how much information to forget from the hidden state given the current input and previous hidden state. The following equations provide the calculations for these gates.

\begin{figure}[H]
\centering
\includegraphics[width=0.55\textwidth]{figs/GNN.pdf}
\caption{A modular design for gated recurrent units. }
\label{fig:GNN}
\end{figure}

\begin{equation}
{z_{t}=\sigma(\mathbf{W_{\mathrm{z}}\mathrm{[h_{t-1},g_{t}])}}}
\end{equation}
\begin{equation}
{r_{t}=\sigma(\mathbf{W_{\mathrm{r}}\mathrm{[h_{t-1},g_{t}])}}}
\end{equation}\\

After calculating how much to update and forget from the hidden state, the new state value can be calculated as over two steps as follows.

\begin{equation}
{\tilde{h}_{t}}=\mathrm{Tanh}(\mathbf{W_{\mathrm{h}}\mathrm{[r_{t} \odot h_{t-1},g_{t}])}}
\end{equation}
\begin{equation}
{h_{t}=(1-\mathrm{z_{t}}) \odot \mathrm{h_{t-1}} + \mathrm{z_{t}} \odot \tilde{h}_{t}}
\end{equation}\\
\noindent where $\sigma(i)=\frac{1}{1+e^{-i}}$ and ${Tanh(u_{i})=(e^{u_{i}}-e^{-u_{i}})/(e^{u_{i}}+e^{-u_{i}})}$ are activation functions.
The first step removes from the hidden state what we need to forget, while the second step adds the needed updates to it.

The previous sequence models deal with one sequence as input, while other sequence modelling tasks would require relating two sequences to each other. For example, in language translation it is required to consider the importance of each token in the first language sequence during translation to the second language. Attention mechanisms \citep{NMT_15,Attention_17} aim at fulfilling this requirement through learning a weight matrix over the hidden states generated by an recurrent encoder model and use it to attention the predictions of a decoder model that generates the second sequence token by token. This mechanism has been used in neural machine translation~\cite{NMT_15} to automatically translate sequences of English language to another languages such as French or German.  

Figure \ref{fig:attention} shows a graphical representation for a encoder-decoder recurrent neural network used in a language translation task from English to French. It can be noticed in the upper left side that the attention mechanism gives the highest weight for the ``I'' token when it generates the first equivalent token in the french language ``Je''.

 \begin{figure}[H]
\centering
\includegraphics[width=0.55\textwidth]{figs/attention.pdf}
\caption{An example for an attention mechanism from a language translation task.}
\label{fig:attention}
\end{figure}
 
Augmenting sequence models with an external memory structure(s), was a successful direction towards processing of long and complex (i.e., in terms of context information) sequences. Memory-augmented Neural Networks (MANNs)~\cite{graves2014neural} is a category of neural networks with an external memory. The external memory structure is generally a matrix containing relevant information to input sequence such as context. At each time step, a MANN uses an attention mechanism to read (i.e., associative retrieval) the most relevant parts from the external memory to the current input for inference. MANNs are more advanced than RNNs when an input is too large to be properly embedded in a fixed-size hidden state vector. MANNs succeeded in many applications including question answering (QA)~\citep{sukhbaatar2015end,kumar2016ask,graves2016hybrid}, healthcare~\citep{hasan2016clinical,le2018dual}, dialogue system~\citep{weston2016dialog} and bioinformatics~\citep{lanchantin2017memory}.

One of the common MANNs architectures is the key-value memory network (KVMN)~\citep{miller2016key}. It represents the context information using two components including the keys and the values. Keys hold embeddings for each context component (e.g., learning skill in a KT task), while values stores the state for each key. Figure~\ref{fig:kvm} shows the KVMN model for a question answering task. 

\begin{figure}[H]
\centering
\includegraphics[width=0.85\textwidth]{figs/KVM.pdf}
\caption{The Key-Value Memory Network model~\citep{miller2016key} }
\label{fig:kvm}
\end{figure}

The KVMN model's workflow goes over three steps: 1) key hashing, 2) key addressing, and 3) value reading. The first step transforms an input sample (e.g., question) into an embedding representation, then, the second step attentions the embedding vector with each key (i.e., context component) to get a read weight vector, finally, it reads context information from the value memory using the read weight to retrieve relevant information to the current input.\\





==> kt_problem.tex <==

\section{THE KNOWLEDGE TRACING PROBLEM}
\label{sec:KT_problem}
\q{(discuss: need some polishing)}
The knowledge tracing (KT) problem can be represented as predicting the likelihood of correctly answering an exercise by the student given her past exercise interaction history~\citep{corbett1994knowledge}. Accordingly, the KT problem can be represented as a prediction problem from a machine learning perspective. The targeted probability of correctly answering an exercise is conditioned on the student's current knowledge state which can be represented in different ways as we are going to explore in the related work section. A mathematical formulation of the KT problem can be represented as follows.
Let $\mathrm{Q}=\left\{ q_{1},\ldots,q_{|Q|}\right\}$ be the set of all distinct question tags %\B{the terms used are different from the ones in the intro. There are a few new terms introduced as well. Suggestion: remove this section and add the formal definition in the intro. The formalisation requires more details as well, it is not clear.} 
in a dataset.  Each  $\mathrm{q_{i}\in Q}$ may have a different level of difficulty, which is not explicitly provided. An \emph{exercise} $\mathrm{x_{i}}$ is a pair $\mathrm{\left(q_{i},y_{i}\right)}$ consisting of a question tag $\mathrm{q_{i}}$ and a binary variable $\mathrm{\mathrm{y_{i}\in\{0,1\}}}$ representing the answer, where $0$ means that $\mathrm{q_{i}}$ is incorrectly answered and $1$ means that $\mathrm{q_{i}}$ is correctly answered. When a student interact with the questions in $\mathrm{Q}$, a history of exercises $\mathrm{X}=\langle \mathrm x_{1},x_{2},\ldots,x_{t-1}\rangle $ undertaken by the student can be observed. Based on a history of exercises $\mathrm{X}=\langle \mathrm x_{1},x_{2},\ldots,x_{t-1}\rangle $, we want to predict the probability of correctly answering a new question at time step $\mathrm{t}$ by the student, i.e., $\mathrm{p_{t}=\left(y_{t}=1|q_{t},\mathrm{X}\right)}$. 

We assume that the questions in $\mathrm{Q}$ are associated with $\mathrm{N}$ Knowledge Components (KCs) $\mathrm{C}$. The \emph{state} of each KC $\mathrm{c^{i}\in C}$ is a random variable describing the mastery level of the student on this KC. At each time step $\mathrm{t}$, the \emph{knowledge state} of a student is modelled as a set of all KC states of the student, each corresponding to a KC in $\mathrm{C}$ at time step $\mathrm{t}$.

It is worth noting that \emph{knowledge components} are often referred to using different terms in the literature such as \q{\emph{skills}~\cite{khajah2014}, \emph{learning concepts}, and \emph{latent concepts}~\cite{SKVMN,zhang2017dynamic}.} In this paper, we use the term \emph{knowledge components}.
